Optimizing the Noise in Self-Supervised Learning: from Importance Sampling to Noise-Contrastive Estimation

Self-supervised learning is an increasingly popular approach to unsupervised learning, achieving state-of-the-art results. A prevalent approach consists in contrasting data points and noise points within a classification task: this requires a good noise distribution which is notoriously hard to specify. While a comprehensive theory is missing, it is widely assumed that the optimal noise distribution should in practice be made equal to the data distribution, as in Generative Adversarial Networks (GANs). We here empirically and theoretically challenge this assumption. We turn to Noise-Contrastive Estimation (NCE) which grounds this self-supervised task as an estimation problem of an energy-based model of the data. This ties the optimality of the noise distribution to the sample efficiency of the estimator, which is rigorously defined as its asymptotic variance, or mean-squared error. In the special case where the normalization constant only is unknown, we show that NCE recovers a family of Importance Sampling estimators for which the optimal noise is indeed equal to the data distribution. However, in the general case where the energy is also unknown, we prove that the optimal noise density is the data density multiplied by a correction term based on the Fisher score. In particular, the optimal noise distribution is different from the data distribution, and is even from a different family. Nevertheless, we soberly conclude that the optimal noise may be hard to sample from, and the gain in efficiency can be modest compared to choosing the noise distribution equal to the data's.

==> 97_trash.tex <==

% \paragraph{Ease of Classification}
% It remains to be understood has the `ease of classification' (how `far' $\pd$ and $\pn$ are from each other) impacts the estimation error of an Energy-Based Model $\pTheta$. Parameterizing the model with a scalar such as the normalization $\Theta = Z$ is probably the simplest setup to study how the estimation error of $\Theta^*$ deteriorates as the classification task gets easier. For example, for $\phi(x) = \log x - x$, the estimation error deteriorates as the noise distribution grows farther from the data distribution as measured by the chi-squared divergence. Different choices of classification loss $\phi$ imply different estimation errors that will be be sensitive to different noise distribution profiles (e.g. tail behavior). Here, the NCE estimation error grows with the Bayes-misclassification error (proof in Appendix~\ref{sec:appendix:nce_normalization_estim_error}). Note in table~\ref{table:normalization_estimation_error} that
% \textbf{`without the sigmoid', the estimation error of NCE would have grown with $\KL(\pd, \pn)$. However, this is \textit{not} the case}.


% \begin{theorem}[Estimation Error] 
%     Given the parameterization of an unnormalized model in \eqref{eq:unnormalized_model} where the energy is known, the estimation error of the (log) normalization is
%     %    
%     \begin{align}
%         \Var[\hat{c}]
%         &=  
%         \ldots
%     \end{align}
% \label{th:estimation_error_normalizaton}
% \end{theorem}
% %
% %
% \begin{table}[!h]
%   \caption{
%   Binary Classification losses for different choices of convex function $\phi$. 
%   }
%   \centering
%   \begin{tabular}{l|ll}
%     \toprule
%     {} & Estimation Error & Optimal noise
%     \\
%     {} & $\mathrm{MSE}(\pn)$ & $\pn^*$
%     \\
%     \midrule
%     InvIS & $\mathcal{D}_{\chi^2}^{*}(\pd, \pn)$ & $\pn^* = \pd$ 
%     \\
%     \midrule
%     Logistic & increasing in & $\pn^* \in \argmax_{\pn} \E_d\sigmoid \left( \log \frac{\nu \pn}{\pd} \right)$
%     \\
%     {} & $\E_d[P(Y=1 | \vx)]$ & $\qquad = \{ \pd \} \quad \text{if } \nu=1$
%     \\
%     \midrule
%     IS & $\mathcal{D}_{\chi^2}(\pd, \pn)$ & $\pn^* = \pd$ 
%     \\
%     \midrule
%     Exponential & \ldots & \ldots 
%     \\
%     \bottomrule
%   \end{tabular}
%   \label{table:normalization_estimation_error}
% \end{table}    


 % A common question to ask is what happens to the asymptotic variance of $\vtheta$ when $\nu = 1$ and the noise is adversarial $p_n = p_d$, i.e when it makes the classification task hardest. \citet{gutmann2012nce} answer that question assuming the model is \textit{normalized}, but what about when the model is \textit{unnormalized} and we extract the marginal asymptotic variance of $\vtheta$? We can now answer this question! When $p_n = p_d$,  $w(\vx) = \frac{1}{2}$ and therefore

 %
    % &=
    % 2
    % \int_{0}^{\infty}
    % |x^2 e^{-2 \theta^*} - 1| \pd
    % \\
    % &=
    % -2
    % \int_{0}^{\exp(2 \theta^*)}
    % (x^2 e^{-2 \theta^*} - 1) \pd
    % +
    % 2
    % \int_{\exp(2 \theta^*)}^{\infty}
    % (x^2 e^{-2 \theta^*} - 1) \pd
    % \\
    % &=
    % \int_{-\infty}^{\infty}
    % (x^2 e^{-2 \theta^*} - 1) \pd
    % -
    % 4
    % \int_{0}^{\exp(2 \theta^*)}
    % (x^2 e^{-2 \theta^*} - 1) \pd
    % \\
    % &=
    % \E_d [x^2 e^{-2 \theta^*} - 1]
    % -
    % 4
    % \int_{0}^{\exp(2 \theta^*)}
    % (x^2 e^{-2 \theta^*} - 1) \pd
    % \\
    % &=
    % -1 + e^{-2 \theta^*} e^{2 \theta^*}
    % -
    % 4
    % \left(
    % e^{-2 \theta^*} 
    % \int_{0}^{\exp(2 \theta^*)}
    % x^2 \pd
    % -
    % \int_{0}^{\exp(2 \theta^*)}
    % \pd
    % \right)
    % \\
    % &=
    % -4
    % \left(
    % e^{-2 \theta^*} 
    % \int_{0}^{\exp(2 \theta^*)}
    % x^2 \pd
    % -
    % \int_{0}^{\exp(2 \theta^*)}
    % \pd
    % \right)
% \end{align}
% %
% We now use well-known identities which relate the gaussian integrals to the erf function
% %
% \begin{align}
%     \int x^2 \pd(x)
%     &=
%     2^{-5/2} e^{2 \theta^*} \mathrm{erf}(e^{-\theta^*} x)
%     - 2^{-3/2} \pi^{-1/2} e^{\theta^*} x \exp(-e^{-2\theta^*} x^2)
%     \\
%     \int \pd(x)
%     &=
%     2^{-3/2} \mathrm{erf}(e^{-\theta^*} x)
% \end{align}
% %
% to evaluate
% %
% \begin{align}
%     \E_d 
%     [| g(\vx) |]
%     &=
%     -4
%     \left(
%     e^{-2 \theta^*} 
%     \int_{0}^{\exp(2 \theta^*)}
%     x^2 \pd
%     -
%     \int_{0}^{\exp(2 \theta^*)}
%     \pd
%     \right)
%     \\
%     &=
%     -4
%     \left(
%     2^{-5/2} \mathrm{erf}(e^{\theta^*})
%     -2^{-3/2} \pi^{-1/2} e^{\theta^*} \exp(-e^{2\theta^*})
%     - 2^{-3/2} \mathrm{erf}(e^{\theta^*})
%     \right)
%     \\
%     &=
%     \mathrm{erf}(e^{\theta^*})(2^{1/2} - 2^{-1/2})
%     +
%     e^{\theta^*} \exp(-e^{2\theta^*})
%     2^{1/2} \pi^{-1/2}
% \end{align}
% %

% We can finally write the MSE gap
% %
% \begin{align}
%     \Delta \mathrm{MSE} 
%     &= 
%     \frac{1}{2T} 
%     \big(
%     1 - 
%     \frac{1}{2}
%     \E_d 
%     [| g(\vx) |]
%     ^2 
%     \big)
%     \\
%     &=
%     \frac{1}{2T} 
%     \left(
%     1 - 
%     \frac{1}{2}
%     \big(
%     \mathrm{erf}(e^{\theta^*})(2^{1/2} - 2^{-1/2})
%     +
%     e^{\theta^*} \exp(-e^{2\theta^*})
%     2^{1/2} \pi^{-1/2}
%     \big)
%     ^2 
%     \right)
% \end{align}
% %

%
% \begin{table}[!h]
%   \caption{
%   $\phi$-divergences between normalized distributions and their Bregman generalization to unnormalized distributions. 
%   }
%   \centering
%   \begin{tabular}{l|lll}
%     \toprule
%     Name & Hyperparameter & $\phi$-divergence~\footnote{up to a scaling and constant} \\
%     {} & $\phi(x)$ & $\mathcal{D}_{\phi}(\pd, \pmodel)$ \\
%     \midrule
%     rev-KL & $-1 -\log(x)$ & $\E_{m} \log \frac{\pmodel}{\pd}$ \\
%     \midrule
%     JS & $x\log x - (1+x)\log(1+x)$ & $\mathcal{D}_{KL}(\pd, \frac{\pmodel}{\pd + \pmodel}) + \mathcal{D}_{revKL}(\pd, \frac{\pmodel}{\pd + \pmodel})$ \\
%     \midrule
%     KL & $x \log x - x$ & $\E_{d}  \log \frac{\pd}{\pmodel}  \\
%     \midrule
%     ? & $-2 \sqrt{x}$ & $-\E_m \sqrt{\frac{\pd}{\pmodel}}$ \\
%     \midrule
%     Power & $\frac{1}{1 + \beta} x^{\beta + 1}, \beta > 1$ & $\E_m (\frac{\pd}{\pmodel})^{1 + \beta}$ \\
%     \midrule
%     Harmonic & $\frac{1}{1 + x}$ & $-\E_d \frac{\pmodel}{\pd + \pmodel}$ \\
%     \bottomrule
%   \end{tabular}
%   \label{table:classification_loss_generic}
% \end{table}    

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=\columnwidth]{img/mse_energy_marginal.pdf}
% \caption{Estimation error tradeoff between the energy and normalization. The data distribution is a standard two-dimensional Gaussian distribution, parameterized by (the log-Cholesky factorization of) its covariance matrix. The noise distribution equals the data distribution.
% }
% \label{fig:msevsnoiseval}
% \end{figure} 

%  % NCE recovers Importance Sampling estimators: family
% In fact, connection between the NCE family of estimators and Importance Sampling extends even further. ~\citet{meng1996importancesamplingext} proposes a generalized family of Importance Sampling estimators which has motivated important algorithmic developments such as path sampling~\citep{gelman1998importancesamplingext}. This family of estimators is defined by a generic reweighing $\alpha(\vx)$ of the ratio
% %
% \begin{align}
%     \hat{Z} 
%     &= 
%     \frac{\E_n [f(\vx) \alpha(\vx)]}
%     {\E_d [\pn(\vx) \alpha(\vx)]}
%     =
%     \argmin_{Z} 
%     Z \,\, 
%     \E_d [\pn \alpha]
%     + 
%     Z^{-1} \,\, 
%     \E_n [f \alpha]
% \end{align}
% %
% which we rewrote as the minimizer of a loss to highlight the connection with~\eqref{eq:gnce_bregman_ratio}. For example, $\alpha = \pn^{-1}$ recovers the Importance Sampling estimator. 

% Different values of the classification loss identified by $\phi$ recover well-known estimators of the normalization.
% %
% \begin{table*}[!h]
%   \caption{
%   Binary Classification losses for different choices of convex function $\phi$ recover a family of Importance Sampling estimators for the normalization $Z$.
%   }
%   \centering
%   \begin{tabular}{l|ll}
%     \toprule
%     Name & Classification Loss & Estimator
%     \\
%     {} & $\mathcal{L}(Z; \phi)$ & $Z = \argmin \mathcal{L}(Z)$
%     \\
%     \midrule
%     revKL & $-Z \E_{d} \frac{\pn}{f} + \log Z$ & $\left( \E_d \frac{\pn}{f} \right)^{-1}$
%     \\
%     \midrule
%     JS & $\E_{d} \log \sigmoid \left( \log \frac{f}{\nu Z \pn} \right) + \E_{n} \log \sigmoid \left( \log \frac{\nu Z \pn}{f} \right)$ & implicit
%     \\
%     \midrule
%     KL & $\log Z^{-1} -Z^{-1} \E_{n} \frac{f}{\pn}$ & $\E_n \frac{f}{\pn}$
%     \\
%     \midrule
%     Exponential & $Z^{\frac{1}{2}} \E_d \sqrt{\frac{\pn}{f}} + Z^{\frac{-1}{2}} \E_n \sqrt{\frac{f}{\pn}}$ & $\E_n \sqrt{\frac{f}{\pn}} \left(\E_d \sqrt{\frac{\pn}{f}}\right)^{-1}$
%     \\
%     \midrule
%     Power & $\nu^{-\beta} \left( -Z^{-\beta} \E_d (\frac{f}{\pn})^{\beta} + \frac{\beta}{1 + \beta} Z^{-\beta - 1} \E_n (\frac{f}{\pn})^{1 + \beta} \right)$ & $\E_n (\frac{f}{\pn})^{1 + \beta} \left(\E_d (\frac{f}{\pn})^{\beta} \right)^{-1}$
%     \\
%     \midrule
%     Harmonic & $\E_d \sigmoid \left( \log \frac{\nu Z \pn}{f} \right)^2 + \nu \E_n \sigmoid \left( \log \frac{f}{\nu Z \pn} \right)^2$ & implicit \\
%     \bottomrule
%   \end{tabular}
%   \label{table:gnce_normalization}
% \end{table*}    
% %
% The forward and reverse $\mathrm{KL}$ classification losses recover the Importance Sampling and Inverse Importance Sampling estimators of $Z$. The exponential loss recovers the product of these estimators, which the power loss re-exponentiates. More generally, each of these NCE estimators can be thought of as having a budget of noise samples $\vx_{1:T_n} \simiid \pn$ and data samples $\vx_{1:T_d} \simiid \pd$ (for example using MCMC on the unnormalized $f$), which it converts into an estimate of the partition function by solving a classification task. \textit{NCE therefore generalizes a family of Importance Sampling methods to Energy-Based Models}, where each classification loss yields a different classifier.

% %
% \begin{align}
%     \hat{Z}
%     &=
%     \arg\min_{Z}
%     \nu \E_n
%     \bigg[
%     S_0
%     \bigg(
%     \frac{p(\vx; Z)}{\nu p_n}
%     \bigg)
%     \bigg]
%     -
%     \mathbb{E}_d
%     \bigg[
%     S_1
%     \bigg(
%     \frac{p(\vx; Z)}{\nu p_n}
%     \bigg)
%     \bigg]
%     \enspace .
% \end{align} 
% %
% Both  are defined by a functional hyperparameter, $\alpha$ and $\phi$ respectively. 

% Different choices of $p^{+}$ and $p^{-}$ have been considered in the literature. For example, it is common in Natural Language Processing~\citep{mikolov2013nce,mnih2012condnce} to choose $p^{+}$ as the joint occurrence of two words and the contrast $p^{-}$ as their independent occurrence.
% Arguably, the simplest scenario for inference is to take the data distribution for the positive label $p^{+} = \pd$, and a noise distribution for the negative label $p^{-} = \pn$~\citep{gutmann2012nce}.


% Information theory information-theoric perspective formalizes this connection to classification, by rewriting the loss explicitly as a divergence between the optimal and model classifiers.


% An information-theoric perspective formalizes this connection to classification, by rewriting the loss explicitly as a divergence between the optimal and model classifiers~\citep{pihlaja2010nce,gutmann2011bregman,uehara2018nce}.
% Specifically, a Bregman divergence is used: whereas many divergences used in Machine Learning (\textit{e.g.} $\phi$-divergences or Integral Probability Metrics) require normalized distributions, a Bregman divergence does not. This makes it an ideal choice for comparing classifiers (exponentiated, for positivity, so we end up manipulating the density ratio), which are positive unnormalized distributions.   

% Here, the logistic loss in~\eqref{eq:logistic_loss} can be equivalently written as a Bregman divergence between the optimal and model classifiers~\citep{menon2016nce}
% %
% \begin{align}
%     \mathcal{L}(F)
%     &= 
%     % \nu \E_n 
%     \mathcal{D}_{\phi} \big(
%     \exp(F^*)
%     % \frac{\pd}{\nu \pn}
%     , 
%     \exp(F)
%     % F
%     \big)
%     \\
%     &=
%     \nu \E_n
%     \bigg[
%     S_0
%     \bigg(
%     \exp(F)
%     % \frac{p_\Theta}{\nu p_n}
%     \bigg)
%     \bigg]
%     -
%     \mathbb{E}_d
%     \bigg[
%     S_1
%     \bigg(
%     \exp(F)
%     % \frac{p_\Theta}{\nu p_n}
%     \bigg)
%     \bigg]
%     +
%     \mathrm{constant}
%     \label{eq:gnce_bregman_ratio}
% \end{align} 
% %
% % \begin{align}
% %     \mathcal{L}(F)
% %     &= 
% %     (1 + \nu) \E_{\vx \sim P(\vx)} 
% %     \mathcal{D}_{\phi} \left(
% %     \sigmoid \circ F^*(\vx), \sigmoid \circ F(\vx)
% %     \right)
% %     \label{eq:gnce_bregman_classifier}
% % \end{align} 
% % %
% These two views, in terms of $\phi$ or $(S_0, S_1)$, are equivalent: 
% %
% \begin{align}
%     S_0(x) &= -\phi(x) + \phi'(x)x  
%     \\
%     S_1(x) &= \phi'(x)
% \end{align}
% %
% and
% %
% \begin{align}
%     \phi(x) &= S_1(x) x - S_0(x)
%     \enspace .
% \end{align}
% %
% These simply represent different hyperparameters: $\phi$ is a convex function while $(S_0, S_1)$ are two nonlinearities that are bound by the relationship $\frac{S_0^{'}}{S_1^{'}}(x) = x$ and $S_1^{'}(x) > 0$.

% The gradient of the classification loss is
% %
% \begin{align}
%     \nabla_{\vTheta} \mathcal{L}(\vTheta)
%     % &=
%     % \nu \E_n 
%     % \bigg[
%     % \frac{p_{\vTheta}}{\nu \pn}
%     % \frac{\nabla_{\vTheta}
%     % p_{\vTheta}}{\nu \pn}
%     % \phi^{''} \big(
%     % \frac{p_{\vTheta}}{\nu \pn}
%     % \big)
%     % \bigg]
%     % -
%     % \E_d
%     % \bigg[
%     % \frac{\nabla_{\vTheta}
%     % p_{\vTheta}}{\nu \pn}
%     % \phi^{''} \big(
%     % \frac{p_{\vTheta}}{\nu \pn}
%     % \big)
%     % \bigg]
%     % \\
%     &=
%     \nu \E_n 
%     \bigg[
%     \nabla_{\vTheta} 
%     \log p_{\vTheta}
%     \bigg(
%     \frac{p_{\vTheta}}{\nu \pn}
%     w
%     \bigg)
%     \bigg]
%     -
%     \E_d
%     \bigg[
%     \nabla_{\vTheta} \log p_{\vTheta}
%     \bigg(
%     w
%     \bigg)
%     \bigg]
%     \label{eq:gnce_gradient}
%     \enspace .
% \end{align}

% The reason for this terminology is that when the model $\pmodel$ is an unnormalized model parameterized by the normalization only, the traditional Importance Sampling and Inverse Importance Sampling Estimators are recovered, as shown in Appendix~\ref{XXX}. Hence, the ``Importance Sampling" and ``Inverse Importance Sampling" classification losses in table~\ref{table:classification_loss_generic} can be seen as generalizing these estimators of the partition function, to estimators for a more general unnormalized model. 

% Note that the Bregman formulation of the NCE loss in \eqref{eq:gnce_bregman_classifier} involves integration with the weighted marginal distribution $(1 + \nu) P(\vx)$ where $P(\vx) = \frac{1}{1 + \nu} (\pd + \nu \pn)$ which is also the mixture distribution between data and noise. Details are available in Appendix~\ref{sec:appendix:nce_bregman_formulation}. 


% \omar{Connection stops here (cf intro)}

% By doing this, we highlight a connection with NCE, also defined as a zero to the gradient of the classification loss as in~\eqref{eq:gnce_bregman_ratio}
% %
% \begin{align}
%     \nabla_{\vTheta} \mathcal{L}(\vTheta)
%     &=
%     Z^{-1}
%     \E_d [w]
%     - \nu Z^{-2}
%     \E_n 
%     \bigg[
%     \frac{f}{\nu \pn}
%     w
%     \bigg]
%     \enspace .
% \end{align}
% %
% using that $\nabla_{Z} \log p(\vx; Z) = \frac{-1}{Z}$. In fact, the Importance Sampling family and the NCE family of estimators perfectly coincide when the task is balanced $\nu=1$ and when their respective reweighing functions, $\alpha(\vx)$ and $w(\vx)$, differ by a specific multiplicative factor
% %
% \begin{align}
%     \alpha(\vx) 
%     &= 
%     w(\vx) \frac{\nabla_{Z} \log p(\vx; Z)}{\pn(\vx)}
%     \label{eq:connection_is_nce}
%     \enspace .
% \end{align}
% %


% \begin{align}
%     \hat{Z} 
%     &=
%     \argmin_{Z} 
%     Z \,\, 
%     \E_d [\pn \alpha]
%     + 
%     Z^{-1} \,\, 
%     \E_n [f \alpha]
%     \enspace .
% \end{align}
% %
% by pushing $Z$ inside the expectation and recognizing that $\pTheta[\vx] = \frac{f(\vx)}{Z}$ and $\nabla_{\Theta} \log \pTheta[\vx] = \frac{-1}{Z}$. 
% Many estimators are solutions of an optimization problem: this allows them to be defined \textit{implicitly} which allows greater flexibilitys t% In the case where the data model is mis-specified, it is clear what the estimator does. Because the loss is precisely a divergence between the optimal and model classifier, the whenever the model parameter $Z$ or more generally $\vbeta$ (and by extension the model classifier) lives in a constrained space, the minimization defines a projection of the optimal classifier onto that space. 


% If this identity does not hold, which means that the reweighing schemes $\alpha$ or $w$ foregoing any dependency on other hyperparameters (\textit{e.g.} $\pn, \phi$) as in~\citet[Equation 2.3]{meng1996importancesamplingext} or~\citet[Equation 3.24]{uehara2018nce}, 

% . If this identity is satisfied, the Importance Sampling family of estimators of~\citep{meng1996importancesamplingext} can be formulated as a (self-supervised) classification task.
% If the reweighing functions, $\alpha(\vx)$ and $w(\vx)$, are relaxed so that their dependencies on the classification loss in~\eqref{eq:reweighing} are dropped, they generate the same family of estimators (the multiplicative factor can be absorbed in the definition of $w(\vx)$). 


% For example, in the case of estimating Gaussian variance:
% $p^{\mathrm{opt}}_n(x) \propto \frac{1}{\sqrt{2\pi\theta}}e^{-\frac{x^2}{2\theta}}|x^2 - \theta|$
% which is highly \textit{non-Gaussian unlike the data distribution}. Similar derivations can be easily done for the cases of Gaussian mean or correlation.



% %
% \begin{theorem}[Marginal Estimation Errors] 
%     Given the parameterization of an unnormalized model in \eqref{eq:unnormalized_model}, the marginal estimation errors of the energy and log-normalization are
%     %    
%     \begin{align}
%         \Var[\hat{\vtheta}] 
%         &=  
%         \mI_{F_w}(\vtheta^*)^{-1} \\
%         & 
%         - \frac{1 + \nu}{\nu} \left(1 - \E_{\pd}[w] \right) \enspace
%         \mI_{F_w}(\vtheta^*)^{-1}
%         \vm_w(\vtheta^*)
%         \vm_w(\vtheta^*)^\top
%         \mI_{F_w}(\vtheta^*)^{-1} 
%         \\
%         & 
%         - \frac{1 + \nu}{\nu} \E_{\pd}[w]  \left(1 - \E_{\pd}[w] \right) \enspace
%         \vm_w(\vtheta^*)
%         \mI_{F_w}(\vtheta^*)^{-1}
%         \mI_{F_w}(\vtheta^*)^{-1}
%         \vm_w(\vtheta^*)^\top
%         \\
%         \Var[\hat{c}]
%         &=  
%         a(\vtheta^*)
%         - \frac{1+\nu}{\nu} 
%         (\mathbb{E}_{\pd}[w] a(\vtheta^*) - b(\vtheta^*))^2
%     \end{align}
% \label{th:estimation_error_marginals}
% \end{theorem}
% %
% using shorthand notations
% %
% \begin{align}
%     a(\vtheta^*)
%     &= 
%     1 - 
%     \vm_w(\vtheta^*)^\top
%     \mI_{w}(\vtheta^*)^{-1}
%     \vm_w(\vtheta^*)
%     \\
%     b(\vtheta^*) 
%     &= 
%     \vm_w(\vtheta^*)^\top
%     \mI_{F_w}(\vtheta^*)^{-1} 
%     \vm_w(\vtheta^*)
%     \\
%     &= 
%     \vm_w(\vtheta^*)^\top
%     (\mI_{w}(\vtheta^*) - \vm_w(\vtheta^*)\vm_w(\vtheta^*)^\top)^{-1} 
%     \vm_w(\vtheta^*)
%     \enspace .
% \end{align}
% %
% The proof is provided in Appendix~\ref{app:sec:nce_var_marginal}.


% In this work we aim to directly optimize the MSE of the original NCE estimator with respect to the noise distribution.
% Analytically minimizing the $\mathrm{MSE}_{\mathrm{NCE}}$ with respect to the noise distribution $p_n$ is a difficult task: it appears \omar{btw exclusively in the reweighting function} (i) nonlinearly (leading to implicit equations) within the integrands of integrals that will need to be (ii) inversed and/or (iii) timed. 
% Even in the simple case where the data follows a one-dimensional Gaussian distribution parameterized by variance, as specified in Section~\ref{sec:XXX} of the Supplementary Material, the resulting expression for the estimation error is intractable. 

% As a reminder, normalized and energy-based parametric models are built from the above table using \eqref{eq:normalized_model} and \eqref{eq:unnormalized_model}, respectively.
%
% \begin{align}
%     p(x; \theta)
%     &=
%     \frac{\tilde{p}(x; \theta)}{Z(\theta)}
%     \\
%     p(x; \Theta)
%     &=
%     \tilde{p}(x; \theta) \exp(-c)
%     \quad \text{where } \Theta = [\theta, c]^\top
%     \enspace.
% \end{align}


% Learning a parametric model of a data distribution is at the core of statistics and machine learning. Among an arsenal of statistical methods developed for this problem, Maximum-Likelihood Estimation (MLE) has stood out as the go-to method: it evaluates a model's likelihood to have generated data observations, and retains the best fit. However, MLE is limited by the fact that the parametric model has to be properly normalized, which may not be computationally feasible when the normalization constant is unknown~\citep{gutmann2013ebmreview}.

% While MLE is known to be optimal in the asymptotic limit of infinite samples, NCE is a popular choice in practice due to its computational advantage. In fact, NCE outperforms Monte Carlo Maximum Likelihood (MLE-MC) \citep{rioudurand2018nce} - an MLE estimation procedure where normalization is performed by importance sampling. 




% \newpage

% In the above, we have chosen the setting of estimating \textit{normalized} distributions, where the performance of Noise-Contrastive Estimation (NCE), measured by the MSE of the estimated parameter, can be baselined: a lower bound is provided by Maximum-Likelihood Estimation (MLE). This gives us an optimality gap between NCE and MLE. 

% While this setting is pedagogical, it uses the fact that MLE is statistically optimal --- so why use NCE? In practice, the advantage of NCE is its ability to handle the estimation of distributions where the normalization $Z(\theta)$ is not known; these are also called Energy-Based Models (EBM).

% The score is now taken with respect to $\tilde{\theta}$ and therefore contains an extra entry: $\tilde{\vg}(\vx) := \nabla_{\vtheta} \log p_{\tilde{\vtheta}}(\vx) \big|_{\tilde{\vtheta} = \tilde{\vtheta}^*} = [\vg(\vx), 1]^\top$. With this slight modification, \citet{gutmann2012nce} show the parametric error given by the MSE formula in Eq.~\eqref{eq:asympmsence} holds. We show in the Supp. Mat.'s Section~\ref{sec:effectnormalization}. that the non-parametric error given by the KL formula in Eq.~\eqref{eq:avgklerror} similarly holds. 

% Hence, with this modification, our formulae for the optimal noises in Eqs.~\eqref{eq:allnoisebestmse} \eqref{eq:alldatabestmse}~\eqref{eq:allnoisebestkl} \eqref{eq:alldatabestkl} hold using $\tilde{\vg}(\vx)$. The question becomes: how different are these optimal noise distributions when the data model is unnormalized? and how does adding the normalization $Z$ to the (joint) estimation affect the error in $\theta$?
% \textit{This is highly dependent on the scaling in the parameterization of the normalization}. As shown in the Supp. Mat.'s Section~\ref{sec:effectnormalization}, the normalization can be arbitrarily scaled, such that its weight relative to the original term in $\vtheta$ is magnified or diminished. Namely, the optimal noises in Eqs.~\eqref{eq:allnoisebestmse} \eqref{eq:allnoisebestkl} remain unchanged when the normalization term dominates in scale, and converge to the data distribution when the normalization term vanishes in scale. In other hands, how we choose to scale the parameterization of the normalization, defines an interpolation between the optimal noises in the normalized case (from Eqs.~\eqref{eq:allnoisebestmse} \eqref{eq:allnoisebestkl}) and the data distribution. 




% \subsection{Definitions}

% Many machine learning problems can understood from the viewpoint of nonparametric estimation, that is, learning the data distribution $\pd$. This can be typically cast as an optimization problem, where we minimize a divergence between the data distribution $\pd$ and a model distribution $\pmodel$
% %
% \begin{align}
%     \min_{\pmodel} \mathcal{D}(\pd, \pmodel)
%     \enspace .
% \end{align}
% %
% It is common to choose the model distribution $\pmodel = \pbeta$ in a parametric family. Though the endgoal may still be the non-parametric estimation of $\pd$, it recasts an optimization problem over distributions which live in an infinite-dimensional space, into an optimization problem over parameters which live in a finite-dimensional vector space. This is arguably most convenient, algorithmically if not mathematically. Alternatively, the endgoal may be the parametric estimation of $\beta$, for e.g. the mixing matrix in an ICA problem. Minimizing this using finite samples defines an estimator
% %
% \begin{align}
%     \hat{\vbeta} 
%     &= 
%     \arg \min_{\vbeta}
%     \mathcal{D}(\pd, \pbeta)
% \end{align}
% %
% whose statistical properties (\textit{e.g.} bias, variance) are entirely determined by the choice of divergence. 
% %
% \begin{align}
%     \hat{\vbeta} 
%     &= 
%     \arg \min_{\vbeta}
%     \mathcal{D}(\pd, \pbeta)
% \end{align}
% %
% An important class of divergences are based on the density ratio between the two distributions that are compared. These are called $\phi$-divergences and are defined as
% %
% \begin{align}
%     \mathcal{D}_{\phi}(\pd, \pmodel)
%     &= 
%     \E_{\pmodel} 
%     \big[ 
%     \phi \big( \frac{\pd}{\pmodel} \big)
%     \big]
%     \label{eq:fdiv_def}
% \end{align}
% %
% where $\phi$ is a hyperparameter that is a convex function. Different values of $\phi$ recover well-known divergences (\textit{e.g.} Kullback-Leibler, Jensen-Shannon, $\chi^2$) so $\phi$ can effectively be understood as a (functional) hyperparameter that interpolates between different divergences of that family. $\phi$-divergences require however that the two distributions $\pd$ and $\pmodel$ be normalized. This can be circumvented when we require only samples from either of these samples, but if evaluation is required in~\eqref{eq:fdiv_def} this can become problematic. Indeed, an energy-based or unnormalized parameterization of $\pmodel$ is more expressive, thus reducing the mis-specficiation error, so it would be convenient to find a class of divergences that can cope with unnormalized models $\pmodel$. This leads us to Bregman divergences



% This result is immediately obtained by noting in \eqref{eq:asympmsence} that the reweighting becomes as a constant $w(\vx) = P(Y = 1 | \vx) = \frac{\pd}{\pd + \nu \pn} = \frac{1}{2}$ and that the score mean is null for a normalized model. In the same adversarial setting, how does the estimation error compare for a \textit{energy-based} model?


% Recall that in an adversarial classification setting, where the distributions of each class are equal $\pn = \pd$, \citet{gutmann2012nce} note that that normalized models have an estimation error that is $(1 + \frac{1}{\nu})$ times the Cramer Rao Lower Bound $\frac{1}{T}\mathrm{tr}(\Ifisher^{-1})$. \citet{pihlaja2010nce} provides the intuitive explanation that ``the variance in the estimator is caused by sampling from two distribution that are independent from each other". 


% \paragraph{Notation} We denote with $p_d$ a data distribution, 
% $p_n$ a noise distribution, and $(p_{\vtheta})_{\vtheta \in \Theta}$ 
% a parametric family of distributions assumed to contain 
% the data distribution $p_d = p_{\vtheta^*}$. 
% All distributions are normalized, meaning that the NCE estimator does not consider the normalizing constant as a parameter to be estimated to simplify the analysis: in this setup, NCE can be fairly compared to MLE and the Cramer-Rao bound is well-defined and applicable.
% The logistic function is denoted by  $\sigma(x)$. 
% We will denote by $\nu$ the ratio between the number of noise samples and data samples: $\nu = T_n / T_d$.
% The notation $\langle x, y \rangle_\mA := \langle x, \mA y \rangle$ refers to the inner product with metric $\mA$. The induced norm is $\| \vx \|_\mA := \| \mA^{\frac{1}{2}} \vx \|$.


% \paragraph{Relaxing the reweighting and Fisher score} 
% Pushing further, \citet[Definition 3]{uehara2018nce} proposed to relax both the reweighting function and the Fisher score. We rewrite \eqref{eq:nce_implicit_bregman} as 
% %
% \begin{align}
%     0
%     &=
%     \nabla_{\vbeta} 
%     \mathcal{L}(\vbeta)
%     =
%     \nu \E_{\vx \sim \pn}
%     [
%     p_{\vbeta}(\vx)
%     \,
%     \alpha(\vx)
%     ]
%     -
%     \E_{\vx \sim \pd}
%     [
%     \pn(\vx)
%     \,
%     \alpha(\vx)
%     ]    
%     \enspace .
%     \label{eq:nce_implicit_alpha}
% \end{align}
% %
% where $\alpha$ encompasses both the reweighting function $w$ and the Fisher score (or log-likelihood for normalized models)
% %
% \begin{align}
%     \alpha(\vx) 
%     &= 
%     w(\vx) \frac{\nabla_{\vbeta} \log p_{\vbeta}}{\pn}(\vx)
%     \label{eq:connection_is_nce}
%     \enspace .
% \end{align}
% %
% \eqref{eq:connection_is_nce} was considered in~\citet[Equation 22]{xing2022adaptiveIS} in a similar context, without drawing the connection to NCE. Again, departing from the classification framework, \citet[Definition 3]{uehara2018nce} propose to relax NCE using an unconstrained reweighting $\alpha(\vx)$~\footnote{Technically, \citet[Definition 3]{uehara2018nce} considered the function $\vx \rightarrow \alpha(\vx) \pn(\vx)$, which we wrote using $\alpha(\vx)$ for the clarity of our expose.}. 

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=\columnwidth]{img/partition_mse_noise_tail.pdf}
% \caption{Estimation error for different noise profiles (tail behavior).}
% \label{fig:estimation_error_partition}
% \end{figure} 

% family of classification losses --- each one obtained for a different value of $\phi$ (see  table~\ref{table:classification_loss_generic}).
% These two formulations of the Bregman divergence, in terms of $\phi$ or $(S_0, S_1)$, are equivalent. These simply represent different hyperparameters of the Bregman family of losses: $\phi$ is a convex function while $(S_0, S_1)$ are two nonlinearities that are bound by the relationship $\frac{S_0^{'}}{S_1^{'}}(x) = x$ and $S_1^{'}(x) > 0$. 



% % \aapo{The basic definition of a Bregman divergence $\mathcal{D}_{\phi}$ is given by}
% %
% \begin{align}
%     \mathcal{L}(F)
%     &= 
%     % \nu \E_n 
%     \mathcal{D}_{\phi} \big(
%     \exp(F^*)
%     % \frac{\pd}{\nu \pn}
%     , 
%     \exp(F)
%     % F
%     \big)
%     \\
%     &=
%     \nu \E_n
%     \bigg[
%     S_0
%     \bigg(
%     \exp(F)
%     % \frac{p_\Theta}{\nu p_n}
%     \bigg)
%     \bigg]
%     -
%     \mathbb{E}_d
%     \bigg[
%     S_1
%     \bigg(
%     \exp(F)
%     % \frac{p_\Theta}{\nu p_n}
%     \bigg)
%     \bigg]
%     +
%     \mathrm{constant}
%     \label{eq:gnce_bregman_ratio}
% \end{align}
% %

% Different values of $\phi$ recover different classification losses. For example, $\phi(x) = x\log x - (1+x)\log(1+x) $ recovers the \textit{logistic} loss.  Note that for another family of divergences, the Csiszár family, this choice of $\phi$ is associated with the Jensen-Shannon (JS) divergence. By analogy, we will call this the Jensen-Shannon classification loss following~\citet{uehara2018nce}. Another choice, $\phi(x) = (1- \sqrt{x})^2$, recovers the \textit{exponential} loss, associated with the squared Hellinger ($H^2$) classification loss. Two additional choices of $\phi$ will be of interest to us in this manuscript: $\phi(x) = x \log x - x$ associated with the Kullback-Leibler (KL) classification loss and $\phi(x) = -1 -\log(x)$ associated with the reverse-KL classification loss. 
% Further details on how the Bregman divergence is used in this manuscript can be found in Appendix~\ref{app:sec:nce_bregman_formulation}.

% Once a loss is chosen, there simply remains to optimize it. Take for example the logistic classification loss
% which can be interpreted as the log-likelihood for the binary classification task. 
% \begin{align} % multiline
%     \mathcal{L}(F)
%     &= 
%     -\E_d
%     [\log \sigma \circ F(\vx)]
%     -
%     \nu
%     \E_n
%     [\log (1 - \sigma \circ F(\vx))]
%     \enspace .
% \end{align} 
% %
% The (Bayes) optimal classifier is defined by setting the (nonparametric) gradient null
% %
% \begin{align} % multiline
%     0
%     =
%     \delta \mathcal{L}(F)
%     &=
%     -\E_d [
%     1 - \sigmoid(F)
%     ]
%     +
%     \nu \E_n  [
%     \sigmoid(F)
%     ]
%     \\
%     &=
%     -\E_d  \left[
%     P(Y=0|x; F)
%     \right]
%     +
%     \nu \E_n \left[
%     P(Y=1|x; F)
%     \right]
% \end{align} 
% %
% and can be numerically approached by gradient descent steps


% %
% \begin{align}
%     \hat{\vbeta}
%     =
%     \arg\min_{\vbeta}
%     \mathcal{L}(\vbeta)
%     =
%     \nu \E_{\vx \sim \pn}
%     \bigg[
%     S_0
%     \bigg(
%     \frac{p_\beta}{\nu \pn}(\vx)
%     \bigg)
%     \bigg]
%     -
%     \E_{\vx \sim \pd}
%     \bigg[
%     S_1
%     \bigg(
%     \frac{p_\beta}{\nu \pn}(\vx)
%     \bigg)
%     \bigg]
%     % =
%     % \mathcal{D}_{\phi}
%     % \left(
%     % \frac{\pd}{\nu \pn}
%     % ,
%     % \frac{p_\beta}{\nu \pn}
%     % \right)
%     \enspace .
%     \label{th:gnce_bregman_recall}
% \end{align}
% %

% Pedagogical contrib. Correlate samples (reprendre preuve) vs. Rao-Blackwellize pn. 
% Try correlated samples (y=x, pn=pd) and see if efficiency is achieved (no but check how grad var is changed).
% Then check Uehara’s pn estimated from y: 4.30.
% Then both: Uehara’s latest. Efficiency achieved.

% \subsection{Where does the variance come from?}
% Consider the infinite sample NCE loss
% %
% \begin{align}
%     \mathcal{L}(p_{\beta})
%     := 
%     \mathcal{D_{}}
% \end{align}
% %
% : it is a (scaled) Bregman divergence
% b which is a divergence


% \paragraph{Where does the variance come from?}
% Consider the infinite sample NCE loss
% %
% \begin{align}
%     \mathcal{L}(p_\beta)
%     =
%     \nu \E_n
%     \bigg[
%     S_0
%     \bigg(
%     \frac{p_\beta}{\nu \pn}
%     \bigg)
%     \bigg]
%     -
%     \E_d
%     \bigg[
%     S_1
%     \bigg(
%     \frac{p_\beta}{\nu \pn}
%     \bigg)
%     \bigg]
%     =
%     \mathcal{D}_{\phi}
%     \left(
%     \frac{\pd}{\nu \pn}
%     ,
%     \frac{p_\beta}{\nu \pn}
%     \right)
% \end{align}
% %
% Using finite samples introduces implementaibility at the price of variance
% %
% \begin{align}
%     \mathcal{L}(p_\beta)
%     =
%     \nu \E_{n_{\mathrm{emp}}}
%     \bigg[
%     S_0
%     \bigg(
%     \frac{p_\beta}{\nu \pn}
%     \bigg)
%     \bigg]
%     -
%     \E_{d_{\mathrm{emp}}}
%     \bigg[
%     S_1
%     \bigg(
%     \frac{p_\beta}{\nu \pn}
%     \bigg)
%     \bigg]
% \end{align}
% %
% but where exactly does the variance come from? Qualitatively, we may distinguish two sources of variance: 
% %
% \begin{itemize}
%     \item A discrepancy between noise sampling and evaluation

%     “variance is caused by sampling from two distributions that are independent of each other”~\citep{pihlaja2010nce}
% \end{itemize}
% %



% . Indeed, setting the gradient null is then written as
% %
% \begin{align}
%     0
%     &=
%     \nabla_{\vbeta} 
%     \mathcal{L}(\vbeta)
%     =
%     \nu \E_{\vx \sim \pn}
%     \bigg[
%     \nabla_{\vbeta} 
%     \log p_{\vbeta}(\vx)
%     \bigg(
%     \frac{p_{\vbeta}}{\nu \pn}(\vx)
%     w(\vx)
%     \bigg)
%     \bigg]
%     -
%     \E_{\vx \sim \pd}
%     \bigg[
%     \nabla_{\vbeta} 
%     \log p_{\vbeta}(\vx)
%     \bigg(
%     w(\vx)
%     \bigg)
%     \bigg]    
%     \enspace .
%     \label{eq:nce_implicit_bregman}
% \end{align}
% %
% which is the difference of the Fisher score (or log-likelihood for normalized models), computed over a dataset reweighted by
% 
%




% The first strategy is \textit{analytical} and explored in Section~\ref{sec:theoretical_results}. It is possible to study some limit cases, and by means of Taylor expansions, obtain analytical results which hopefully shed some light to the general behaviour of the optimal noise distribution even far away from those limits. 
% The second strategy is \textit{numerical} and found in Section~\ref{sec:numerical_results}. We use a parametric or histogram-based expression for $p_n$ and numerically optimize the MSE with respect to it. 


% \paragraph{Generalization Error}
% It is well-known that the generalization error in the framework of ERM decomposes into three terms~\citep[Introduction to Statistical Learning Theory, Section 2.2]{bousquet2004stattheory}: the approximation error (due to mis-specification), the estimation error (due to finite samples), and the optimization error (due to finite iterations). Among these three, we focus in this manuscript on the estimation error. Theoretically, it conveniently has a clear formula from which we can derive the optimal hyperparameters, \textit{i.e.} those that minimization the estimation error. In practice, we consider that the approximation error of NCE is mitigated by expressive parameterizations~\citep{gao2020fce} of the data model using neural networks, and that the optimization error of NCE is also mitigated using algorithms with adaptive step size~\citep{liu2021nceoptim}, so that the estimation error is left to dominate generalization.


% Importance Sampling is t
% Perhaps the most well-known estimator for $Z$ is given by Importance Sampling~\citep{kahn1949importancesampling,owenmontecarlobook}, defined as
% %
% \begin{align}
%     \hat{Z} = \E_{\vx \sim \pn}
%     \big[ \frac{f(\vx)}{\pn(\vx)} \big] 
%     \enspace ,
% \end{align}
% %

 % Note that, when  $\alpha = \pn^{-1}$ one recovers the original Importance Sampling.
 % Other values of $\alpha$ recover other estimators in this Importance Sampling family, which has motivated important algorithmic developments for estimating $Z$~\citep{gelman1998importancesamplingext}. We re-arrange the equation to write the estimator as the zero of the following equation
% Though the estimator is explicit, it is useful to write it as the minimizer of a loss
%


% We next show it is also possible to shed some light on the behavior of the JS case by studying two important limit cases:
% %
% \begin{enumerate}
% \item The limit of all noise observations: $\nu \rightarrow \infty$, which is common in self-supervised classification literature~\citep{mnih2012condnce,wang2020sslgeometry,chuang2020debiasedinfonce}.
%     \item The limit of all data observations: $\nu \rightarrow 0$. This limit may be less realistic but interesting from a theoretical viewpoint.
    
% \end{enumerate}
% %
% These are the two extreme cases for an unbalanced classification task, when the budget of samples is limited exclusively to one source, noise or data. Using these two limit cases, we prove in Appendix~\ref{app:ssec:limits_motivation} that the JS classification loss
% interpolates between the forward and reverse KL classification losses in the sense that



% loss for the origina the 
% the JS classification loss
% interpolates between the forward and reverse KL classification losses in the sense that

% These are the two extreme cases for an unbalanced classification task, when the budget of samples is limited exclusively to one source, noise or data. Using these two limit cases,  that the JS classification loss
% interpolates between the forward and reverse KL classification losses in the sense that

% This approach has been  estimation methods
% ~\citep{pihlaja2010nce,gutmann2011bregman}
% $\frac{1}{\sqrt{\epsilon}}$ 

%,
%ven when imposing, for example, unit-variance on the data distribution $\alpha=1$.

% \if0
% \aapo{\bf OLD TEXT:}
% In this case, we can write out:

% \begin{itemize}

%     \item the 2D score:
%     $g(x) = 
%     \begin{pmatrix}
%         \frac{1}{\alpha}x \\
%         -\frac{1}{2\alpha} + \frac{1}{2\alpha^2}x^2
%     \end{pmatrix}$

%     \item its pointwise covariance:
%     $g(x)g(x)^\top = 
%     \begin{pmatrix}
%         \frac{1}{\alpha^2}x^2 & -\frac{1}{2\alpha^2}x + \frac{1}{2\alpha^3}x^3 \\
%         -\frac{1}{2\alpha^2}x + \frac{1}{2\alpha^3}x^3 & -\frac{1}{4\alpha^4}x^4 - \frac{1}{2\alpha^3}x^2 + \frac{1}{4\alpha^2}
%     \end{pmatrix}$

%     \item the optimal discriminator:
%     $1 - D(x) = 
%     \frac{\nu \pn(x)}{\nu \pn(x) + \pd(x)}
%     =
%     \frac{1}{1 + \frac{1}{\nu}\sqrt{\frac{\beta}{\alpha}} e^{\frac{-x^2}{2}(\frac{1}{\alpha} - \frac{1}{\beta})}}
%     % \sigma_{\frac{1}{\nu}\sqrt{\frac{\beta}{\alpha}}}(\frac{x^2}{2}(\frac{1}{\alpha} - \frac{1}{\beta}))
%     $
% \end{itemize}

% Now we can compute the (generalized) score mean $\vm$ and covariance $\mI$ as they intervene in the MSE formula for Noise-Contrastive Estimation:

% \begin{align*}
%     \vm & = 
%     \int \nabla_{\vbeta} F(\vx, \vbeta^*) (1 - D(\vx)) p(\vx)d\vx
%     =
%     \begin{pmatrix}
%         m_1 \\
%         m_2
%     \end{pmatrix}
% \end{align*}

% where

% \begin{align*}
%     \begin{cases}
%         m_1 & = 0 \quad \text{(the integrand is an odd function)} \\
%         m_2 & = 
%         -\frac{1}{2\alpha\sqrt{2\pi\alpha}} 
%         \int 
%         \left( e^{\frac{-x^2}{2\alpha}} \frac{1}{1 + \frac{1}{\nu}\sqrt{\frac{\beta}{\alpha}} e^{\frac{-x^2}{2}(\frac{1}{\alpha} - \frac{1}{\beta})}} \right)dx \\
%         & + 
%         \frac{1}{2\alpha^2\sqrt{2\pi\alpha}} 
%         \int 
%         x^2
%         \left( e^{\frac{-x^2}{2\alpha}} \frac{1}{1 + \frac{1}{\nu}\sqrt{\frac{\beta}{\alpha}} e^{\frac{-x^2}{2}(\frac{1}{\alpha} - \frac{1}{\beta})}} \right)dx   
%     \end{cases}
% \end{align*}

% and 

% \begin{align*}
%     \mI & = 
%     \int \nabla_{\vbeta} F(\vx, \vbeta^*)\nabla_{\vbeta} F(\vx, \vbeta^*)^\top (1 - D(\vx)) p(\vx)d\vx
%     =
%     \begin{pmatrix}
%         I_{11} & I_{12} \\
%         I_{21} & I_{22} \\
%     \end{pmatrix}
% \end{align*}

% where 

% \begin{align*}
%     \begin{cases}
%         I_{12} & = I_{21} = 0 \quad \text{(the integrand is an odd function)} \\
%         I_{11} & =
%         \frac{1}{\alpha^2\sqrt{2\pi\alpha}} 
%         \int 
%         x^2
%         \left( e^{\frac{-x^2}{2\alpha}} \frac{1}{1 + \frac{1}{\nu}\sqrt{\frac{\beta}{\alpha}} e^{\frac{-x^2}{2}(\frac{1}{\alpha} - \frac{1}{\beta})}} \right)dx \\ 
%         I_{22} & = 
%         \frac{1}{4\alpha^4\sqrt{2\pi\alpha}} 
%         \int 
%         x^4
%         \left( e^{\frac{-x^4}{2\alpha}} \frac{1}{1 + \frac{1}{\nu}\sqrt{\frac{\beta}{\alpha}} e^{\frac{-x^2}{2}(\frac{1}{\alpha} - \frac{1}{\beta})}} \right)dx \\
%         & - 
%         \frac{1}{2\alpha^3\sqrt{2\pi\alpha}} 
%         \int 
%         x^2
%         \left( e^{\frac{-x^2}{2\alpha}} \frac{1}{1 + \frac{1}{\nu}\sqrt{\frac{\beta}{\alpha}} e^{\frac{-x^2}{2}(\frac{1}{\alpha} - \frac{1}{\beta})}} \right)dx \\
%         & +
%         \frac{1}{4\alpha^2\sqrt{2\pi\alpha}} 
%         \int 
%         \left( e^{\frac{-x^2}{2\alpha}} \frac{1}{1 + \frac{1}{\nu}\sqrt{\frac{\beta}{\alpha}} e^{\frac{-x^2}{2}(\frac{1}{\alpha} - \frac{1}{\beta})}} \right)dx   
%     \end{cases}
% \end{align*}

% Even in a simple 1D Gaussian setting, 
% evaluating the asymptotic MSE of the Noise-Contrastive Estimator is untractable in closed-form,
% given the integrals in $m_2, I_{11}, I_{22}$. While here we considered the case of two parameters, the intractability is seen even if we constrain the analysis to one of them, which would leave us with the diagonal entries $I_{11}$ and $I_{22}$

% Optimizing the asymptotic MSE 
% with respect to $\beta$ (noise distribution) or $\nu$ (identifiable to the noise proportion)
% yields similarly intractable integrals,
% even when imposing, for example, unit-variance on the data distribution $\alpha=1$.


% This could mean assigning a positive label to adjacent points in a timeseries and a negative label to far-away points in a timeseries~\citep{hyvarinen2017pcl,banville2020ssleeg} requires learning features related to the temporal correlation structure~\citep{liu2021condncetimeseries}.


% new theoretical contributions
% 1. Formulae + simulations for EBMs, including the adversarial setting (noise = data)
% 2. Link with Importance Sampling
% 3. Quantifying how the hardness of the classification task (divergence between pn and pd) impacts the density estimation (MSE) 
% 4. Highlighting that for any data distribution, the optimal Pihlaja noise does not bring substantial MSE gain (worth the trouble)


% A statistical approach provides a useful solution. The evaluation dataset is considered to be generated in the same way as the train dataset and with an infinite sample. The classifier is also trained and evaluated using the same cost function. This is the framework of Empirical Risk Minimization (ERM) or M-estimation in statistical parlance. This way, the design of the classification task is removed from the variability of domain-specific datasets that could be used for evaluation. Indeed, the \textit{generalization error} is well-understood in the framework of ERM.

%Once a model is learnt, it can be used to generate new data, to evaluate the likelihood of existing data, or be introspected for meaningful structure such as conditional dependencies between its input features. 

% However, such an adversarial form of training where a noise generator aims to fool the discriminator suffers from instability and mode-collapse \citep{dieng2019gan, lorraine2021complexmomentum}.

%
% Last, by viewing the estimation of the normalization $Z$ as a special case of NCE when the energy-based model has only one unknown only --- the normalization --- we moreover extend the result of~\citet{bennett1976ncepartition} by interpreting the NCE estimator and its optimal hyperparameters through the lens of Markov Chain Monte Carlo (MCMC). This is contained in Appendix~\ref{app:ssec:nce_mcmc} as it is a noteworthy yet peripheral to our main expose.
%


% , which the power loss re-exponentiates. 
%Aapo: repetitive
%More generally, each of these NCE estimators can be thought of as having a budget of noise samples $\vx_{1:T_n} \simiid \pn$ and data samples, $\vx_{1:T_d} \simiid \pd$
% (for example using MCMC on the unnormalized $f$)
%which it converts into an estimate of the normalization by solving a classification task. 

% %
% \begin{enumerate}
%     \item The limit of all noise observations: $\nu \rightarrow \infty$, which is common in self-supervised classification literature~\citep{mnih2012condnce,wang2020sslgeometry,chuang2020debiasedinfonce}.
    
%     \item The limit of all data observations: $\nu \rightarrow 0$. This limit may be less realistic but interesting from a theoretical viewpoint.
%     \enspace .
% \end{enumerate}
% %

% higher variance of the estimator. %Indeed, there are many ways to measure how the noise distribution may ``depart from" the data distribution: there could be a mismatch in the modes, or the moments, or the tails, to cite a few. 
% Different estimators in the NCE family %, defined by different classification losses, 
% are affected by that ``density chasm"~\citep{rhodes2020bridgedre} based on the different divergences just given, thus being sensitive to different types of mismatch. 
% \omar{Namely, this implies that that optimality of the proposal $\pn$ is not systematically measured by its KL divergence to the data, contrary to \omar{what is often assumed out of mathematical / algorithmic convenience} a convenient standard~\citep{chatterjee2015ISsamplesize,cerou2022isoptimalnoise,rubinstein2004crossentbook}.}

% %
% \begin{table*}[!h]
%   \caption{
%   Comparing the estimation error in the NCE family, when the model is parameterized generically \textit{versus} with the scalar $Z$.
%   }
%   \centering
%   \begin{tabular}{ccccc}
%     {} & \multicolumn{2}{c|}{Estimate $Z$} & \multicolumn{2}{c}{Estimate any parametric model}
%     \\
%     \hline
%     Name & Estimation Error & Optimal noise & Estimation Error & Optimal noise
%     \\
%     {} & $\mathrm{MSE}(\pn)$ & $\pn^*$ & $\mathrm{MSE}(\pn)$ & $\pn^*$
%     \\
%     \hline
%     \\
%     revKL & $O (\mathcal{D}^{*}_{\chi^2}(\pd, \pn))$ & $\pd$ & $O (\mathcal{D}^{*}_{\chi^2}(\pd \bullet w_1, \pn))$ & $\pd \bullet w_1$
%     \\
%     {} & {} & {} & Supp. constr. (Th.~\ref{th:alldatabestmse}) & (modes)
%     \\
%     \hline
%     \\
%     JS & $O ((1 - \mathcal{D}_{\mathrm{Ha}}(\pd, \pn))^{-1})$ & $\pd$ & \eqref{eq:asympmsence} & unknown
%     \\ \\
%     \hline
%     \\
%     KL & $O (\mathcal{D}_{\chi^2}(\pd, \pn))$ & $\pd$ & $O (\mathcal{D}_{\chi^2}(\pd \bullet w_2, \pn))$ & $\pd \bullet w_2$
%     \\ \\
%     \hline
%   \end{tabular}
% \label{table:nce_estimation_error}
% \end{table*}    
% %

%this question   in the all noise limit for normalized models, quantifying the decrease it provides in parametric estimation error.
% %
% \begin{figure}[!ht]
% \centering
% \includegraphics[width=0.7\columnwidth]{img/mse_summary.png}
% \caption{Estimation error for the energy term, using the adversarial and optimal noises.}
% \label{fig:estimation_error_partition}
% \end{figure} 
% %


% For energy-based models, one can further ask how the \textit{joint} estimation of the energy and normalization affects the \textit{marginal} estimation of the energy $\vtheta$ and of the log-normalization $c$?
% We unpack the marginal variances for the energy term and the log-normalization term in Appendix~\ref{app:ssec:nce_var_ebm_marginals}. Their tradeoff was also explored by~ \citet[Corollary 4]{uehara2018nce} in the all noise limit. 
% We further show that their individual optimization is generally not well-posed in Appendix~\ref{app:ssec:nce_var_ebm_marginals_optim}.

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=\columnwidth]{img/optimal_noise_gaussian_mean_ebm_dataval_0.0_panel.pdf}
% \caption{Estimation errors of the energy and the log-normalization. 
% The noise minimizes the estimation error of (i) the energy and log-normalization, (ii) the energy only, or (iii) the log-normalization only. In every case, the energy and normalization are jointly estimated. 
% The data distribution is a one-dimensional Gaussian distribution, parameterized by the mean.
% }
% \label{fig:numericalnoise_gaussian_mean}
% \end{figure} 

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=\columnwidth]{img/optimal_noise_gaussian_logvar_ebm_dataval_0.0_panel.pdf}
% \caption{Estimation errors of the energy and the (log) normalization. 
% The noise minimizes the estimation error of (i) the energy and normalization, (ii) the energy only, or (iii) the normalization only. In every case, the energy and normalization are jointly estimated. 
% The data distribution is a one-dimensional Gaussian distribution, parameterized by the log standard deviation.
% }
% \label{fig:numericalnoise_gaussian_logstd}
% \end{figure} 


% It is common to obtain the optimal classifier $F^*(\vx)$ by minimizing 
% % the ERM objective
% %
% \begin{align}
%     \mathcal{L}(F) 
%     &= 
%     \mathbb{E}_{(\vx, y) \sim p(\vx, y)} 
%     \left[ \ell(F(\vx), y) \right]
%     \propto
%     \nu \mathbb{E}_{\vx \sim \pn} 
%     \left[ \ell(F(\vx), 0) \right]
%     +
%     \mathbb{E}_{\vx \sim \pd} 
%     \left[ \ell(F(\vx), 1) \right]
% \end{align}
% %
% where $\ell$ is a suitable loss function and $\nu=P(Y=0)/P(Y=1)$ denotes the noise to data ratio, also known as the prior odds ratio. 



% \aapo{Note that while we considered above the general case of a non-parametric classifier, in practice it is often parameterized by a finite number of parameters, for example, as a neural network. A parametric classifier then corresponds to a parametric model, as will be considered in detail later.}
%While we estimate a parameter, the end goal could either be parametric or non-parametric. In the former case, it is common to estimate a parametric embedding of the data into a latent space of features, using this self-supervised task~\citep{hyvarinen2017pcl,hyvarinen2019gcl,li2021sslhsic}. In the non-parametric case, the parameters are simply a means to an end: modeling the data distribution. 

 % In practice, we consider that the approximation error of NCE is mitigated by expressive parameterizations~\citep{gao2020fce} of the data model using neural networks, and that the optimization error of NCE is also mitigated using algorithms with adaptive step size~\citep{liu2021nceoptim}, so that the estimation error is left to dominate generalization.
